How do developers discuss and support new programming languages in technical Q&A site? An empirical study of Go, Swift, and Rust in Stack Overflow

New programming languages (e.g., Swift, Go, Rust, etc.) are being introduced to provide a better opportunity for the developers to make software development robust and easy. At the early stage, a programming language is likely to have resource constraints that encourage the developers to seek help frequently from experienced peers active in QA sites such as Stack Overflow (SO). In this study, we have formally studied the discussions on three popular new languages introduced after the inception of SO (2008) and match those with the relevant activities in GitHub whenever appropriate. For that purpose, we have mined 4,17,82,536 questions and answers from SO and 7,846 issue information along with 6,60,965 repository information from GitHub. Initially, the development of new languages is relatively slow compared to mature languages (e.g., C, C++, Java). The expected outcome of this study is to reveal the difficulties and challenges faced by the developers working with these languages so that appropriate measures can be taken to expedite the generation of relevant resources. We have used the LDA method on SO's questions and answers to identify different topics of new languages. We have extracted several features of the answer pattern of the new languages from SO to study their characteristics. These attributes were used to identify difficult topics. We explored the background of developers who are contributing to these languages. We have created a model by combining Stack Overflow data and issues, repository, user data of GitHub. Finally, we have used that model to identify factors that affect language evolution. We believe that the outcome of our study is likely to help the owner/sponsor of these languages to design better features and documentation. It will also help the software developers or students to prepare themselves to work on these languages in an informed way.

==> Sections/Methodology.tex <==
\section{Methodology}
\label{sec:methodology}
\subsection{Selection of the languages}
From Stack Overflow data, we have calculated the number of posts, number of questions and number of answers, and accepted answers along with their percentage among the total number of posts, total number of questions, total number of answers and accepted answers in SO. For  selecting the language, we have used the SO survey~\citep{StackoverflowSurvey} and the newly released language list~\citep{wiki:Timeline}. Most of the new languages (released after 2008) have a little footprint in SO that are not sufficient to formally analyze the evolution of that language. Thus we have picked the top three (considering the number of posts) newly released language for our study. In Table~\ref{table:language stats}, we show the footprints of the languages in SO. To do the comparative analysis with three new languages, we picked one heavily encountered language (Java) and one medium footprint language (Python) to compare the evolution of newly released languages. Since JavaScript is used for web clients only, and Java has a wide range of use, we preferred it as a top-tier language. From the mid-category languages, Python is selected as an emerging language.
\input{Tables/language_stats.tex}
% Table \ref{table:language stats} presents the number of posts, questions, answers and their percentage with respect to total number of SO posts, questions and answers.

\subsection{Data Extraction}

The following steps are followed to develop the dataset for this study.

\begin{enumerate}
    \item \textbf{Download Stack Overflow dataset:} For our analysis, we have collected the December 2017 Stack Overflow data dump which is available in the Stack Exchange data dump. In Stack Overflow schema, both question and answer are considered as \emph{post}. The post table of the data dump contains all the information of a post like a title, tags, body, creation date, view count, type (question or answer) and accepted answer identifier. An answer is accepted if the questioner marks that answer as accepted. Our dataset includes 4,17,82,536 questions and answers posted over some time of over 9 years from August 2008 to December 2017 by 39,40,962 users of Stack Overflow. Among these posts 1,63,89,567 (39\%) are questions and 2,52,97,926 (61\%) are answers of which 87,04,031 (21\%) are marked as accepted answers.
    
 
    \item \textbf{Develop tag set:} To compare the growth of languages, we have to separate the posts by language. Posts on Stack Overflow can be about any topic, we need a way to identify posts by language. Every Stack Overflow post is associated with at least one tag. We consider a post is associated with one of the new languages if that contain at least one tag of tag set of that respective language. We have created an initial set of tag $\uptau_0$ for each language by manually inspecting the tag table of Stack Overflow schema. Next, we go through the Stack Overflow dataset $\mathcal{S}$ and extract questions $\rho$ whose tags contain a tag from  $\uptau_0$. Third, we extract tags of the posts in $\uprho$ to form the set of candidate concurrency tags $\uptau$. Now we have a set of tag $\uprho$ for each language which includes all tags of that language.However, set $\uprho$ may include tags which may be irrelevant to new languages. So following the  approach of Rosen et al.~\citep{Rosen2015} we have  used two heuristics $\alpha$ and $\beta$ to find the the significantly relevant tags for each language. 
    
    \begin{equation}
        \alpha = \dfrac{number \ of \ posts \ with \ tag \ t \ in \ \uprho}{number \ of \ posts \ with \ tag \ t \ in \ \mathcal{S}}
    \end{equation}
    \begin{equation}
         \beta = \dfrac{number \ of \ posts \ with \ tag \ t \ in \ \uprho}{number \ of \ posts \ in \ \uprho}
    \end{equation}

    We have experimented with a broad range of $\alpha$ and $\beta$  and found that $\alpha = 0.01$ and $\beta=0.01$ provides a significantly relevant set of tags. The tagset used to extract posts i this study is available at GitHub.Relevant tags selected for this study is presented in appendix ~\ref{appendix:tagrelevance}. https://git.io/JTIqL

% To compare the growth of languages, we have to separate the posts by language. Every Stack Overflow post is associated with at least one tag. We consider a post is associated with one of the new languages if that contain at least one tag of tag set of that respective language. To develop a set of tag for each language, we have used keywords to search in the tag table and then by manual inspection we have identified relevant tags for each language. 
    
    \item \textbf{Extract posts of new languages:} Using the tag set prepared in the previous step, we have separated the posts by language. We have 4,37,880 Swift posts, consisting of 1,88,065 (43\%) questions and 2,49,815 (57\%) answers of which 94,310 (21.6\%) are accepted answers. We have 72,843  Go posts, consisting of 30,286 (41.6\%) questions and 42,557 (58.4\%) answers of which 19,178 (26.3\%)  are accepted answers. We have 18,311 Rust posts, consisting of 8,083 (44.1\%) questions and 10,228 (55.9\%) answers of which 5,964 (32.6\%) are accepted answers. 

     \item \textbf{Data extraction from GitHub:} GitHub provides access to data of public repositories and users through API\footnote{https://developer.github.com/v3/}. The new languages have their official repository in GitHub. We have collected the creation date and closing date of the issues from the official repositories of these new languages. GitHub issues have two states `open' and `closed.' As soon as an issue is taken care of, it changes its state from `open' to `closed.' Along with the frequency of issues, we have also collected the states of issues. Besides, we have collected the number of users and repositories of each new language.
\end{enumerate}

\iffalse

 \item \textbf{Preprocessing of posts for topic modeling:} To avoid noise, we preprocess the post before topic modeling~\citep{Barua2012}. First, all the codes enclosed in <code> tags, HTML tags, and url are removed. Second, the Porter stemming algorithm~\citep{Porter1997} is applied to convert the words into their base form. Third, all the articles and stop words are removed. Now, the posts are ready for topic modeling. We have used Latent Dirichlet Allocation (LDA)~\citep{Blei2003} to infer topics automatically.
 
 
 
 Stack Overflow publishes its data periodically. We have collected the Stack Overflow data dump in  October 2018. There are total 38485046 posts(both question and answer) in that dump. Stack Overflow posts are associated with tags. Though the tags are added by the users, in the moderation process correct tags will be associated with that post. To separate the posts by languages, we rely on tags. We carefully curated a tag set for each of these languages based on keywords, frameworks etc. from the tag table of Stack Overflow.

GitHub provides access to public data of repository and user through API\footnote{\url{https://developer.github.com/v3/}}. By using that API we have collected information about the official Go, Rust and Swift repository, the number of users and number of repositories of each language.
\fi

==> Sections/OldIntroduction.tex <==
\section{Introduction}
\label{sec:introduction}
New programming languages are being introduced to make software development easy, maintainable, robust, and performance-guaranteed. For example, Swift was introduced in June 2014 as an alternative to Objective-C to achieve better performance. At the initial stage of its lifetime, a programming language is likely to have constraints of resources, and consequently, developers using these languages face additional challenges. Naturally, the developers seek help from community experts of question-answering (QA) sites such as Stack Overflow (SO). Hence, it is expected that the discussions on issues related to a new language in SO represent the different characteristics of the growth of that language and also reflect the demands of the development community who use that language. 

After the release of a new programming language, it takes time for the developers to get acquainted with that language. Earlier releases of new languages often contain bugs. The developers who work on the new languages are likely to face problems that are similar to the solved problems of mature languages. Developers of the new languages often feel the absence of a library or feature that has already been available in other languages. Therefore, the discussions on a new language are likely to differ from that of a mature language. To the best of our knowledge, there is yet to be any software engineering research that focuses on the specific characteristics of the new languages by mining relevant discussions from SO.
%%Detailed knowledge of the growth of resources of a new language can help prevent these issues from appearing again for another language. It is also possible that low-quality documentation and absence of resources in question-answer (QA) sites make the skill growth of developers of new languages slower. 

In this study, we would like to fill this gap, analyzing the discussions on Swift, Go, and Rust that are the most popular programming languages introduced after the inception of SO (2008). Our study is limited to these three languages because other new languages have very small footprints in SO. Being born after SO, the evolution of these languages, right from the beginning, is expected to be reflected in SO. From now on, by the \emph{new language}, we imply Swift, Go, and Rust languages. We also match the SO discussions with the relevant activities in GitHub in the required cases. 

We published partial results of the study in a recent publication~\cite{Chakraborty2019}, which explored three of the seven research questions. All the questions in the previous publication were focused on the availability of solutions. On the other hand, this publication explores the different perspectives of the evolution of new languages (e.g., topics of discussion, evolution, and difficulties, developers' activity, and relationship with the evolution of language).

The primary goal of this research is to study how software developers
discuss and support three new programming languages (Go, Swift, Rust) in Stack
Overflow. On this goal, we conduct two studies:
(1) Understanding New Language Discussions: We aim to understand what topics developers 
discuss about the three new programming languages, whether and how the topics are similar and/or different across 
the languages, and how the topics evolve over time. (2) Understanding New Language Support: We aim to understand  
what difficulties developers face while using the three new languages, and when and how adequate resources and expertise 
become prevalent to support the three new programming languages in Stack Overflow. In particular, we answer seven 
research questions around the two studies as follows. 

\begin{itemize}[leftmargin=10pt]
  \item \textbf{Study  1. New Language Discussions}: We answer two research questions:
  \begin{enumerate}[label={\textbf{RQ\arabic{*}.}}]
    \item \textbf{What are the topics of discussions related to Swift, Go, and Rust?}
    
    This investigates the discussion topics of the developers of new languages. Identification of the discussion topics may help the sponsor to design a feature roadmap that actually facilitates the requirement of developers.
    
    \item \textbf{How do the discussed topics evolve over time?}
    
    The community’s discussion topics is likely to vary over time, as resources evolve continuously.  This analysis would enable us to investigate any possible relation between discussion topics and real-world dynamics, such as new releases.
    
  \end{enumerate}
  \item \textbf{Study 2. New Language Support}: We study the support the three new languages based on two themes (T).
  \begin{description}
  
  \item[- Theme 1. Solution Availability.] We study the difficulty of getting answers. We answer three research questions.
  \begin{enumerate}[label={\textbf{RQ\arabic{*}.}},start=3]
    \item \textbf{How does the difficulty of the topics vary across the languages?}
    
    Developers of new languages face problems that are rarely answered or get \emph{delayed answers}. By the \emph{delayed answer}, we imply that answer which is accepted by the user and received after the median answer interval of that month. We want to know about these questions so that special measures can be taken to answer this question. We found that questions related to migration, data and data structure are considered as difficult topics in all three languages.
    
    \item \textbf{When were adequate resources available for the new programming languages in Stack Overflow?}
    
      In this research question, we want to know the time interval, after which we can expect the availability of these resources of new languages in Stack Overflow at a satisfactory level. The use of programming languages is significantly related to the availability of resources of those languages. This question will help developers to make design decisions related to software development. We have seen that two years after the release, sufficient resources can be expected for Swift, whereas this period is three years for Go. We have also found the evidence of having an inadequate resource of Rust language in Stack Overflow.


    \item \textbf{What are the characteristics of answer pattern for the languages?}
    
    With the evolution of a new language, the number of skilled developers increases. In this question, we wanted to observe the effect of a growing number of skilled developers on answer characteristics such as the expected interval of first and accepted answers, unanswered question ratio. One of the findings of this question is, in Stack Overflow, the unanswered question ratio increases regardless of the age of the language.
\end{enumerate}

     \item[- Theme 2. Developer Engagement.] We study how developers of new languages are engaged. We answer two research questions. 
      \begin{enumerate}[label={\textbf{RQ\arabic{*}.}},start=5]
    \item \textbf{How likely are the questions of the three new languages answered by the developers of predecessor languages?}
    
    Stack Overflow includes developers from a diverse domain. We are interested to see if there is a pattern that the experts in the predecessor of a new language mostly answers the questions of that language (e.g., Objective-C for Swift). This support from predecessor language can help new language developers in the early stages of that particular language. We have seen that the new language receives a significant amount of support from the predecessor language community.

    \item \textbf{Is there any relationship between the growth of the three programming languages and developers' activity patterns?}
    This question investigates the relationship between developers' activity  (e.g.,  question,  answer)  and the growth of a  language. Language projects maintain a Github repository that supports feature requests~\citep{Bissyande2013} and bug reports through  Github issues.  We used those issues as an indirect measure for language growth in this language. We have found evidence of a relationship between developers' activity and the growth of a language.
    \end{enumerate}

  \end{description}
  
\end{itemize}

The major findings of the study are: (i) migration, data and data structure are generally the difficult topics of new languages, (ii) the time when adequate resources are expected to be available vary from language to language, (iii) the unanswered question ratio increases regardless of the age of the language, (iv) a new language is benefited from its predecessor language, and (v) there is a relationship between the developers' activity pattern and the growth of the relevant language.

The motivation behind investigating the first four and sixth research questions is to help the owner/sponsor of these languages design better features and documentation, which would eventually benefit the developers. The general software developers or students can have insight about how to prepare themselves to work on these languages. Moreover, the fifth and seventh research questions would cater to researchers' academic interest by presenting interesting parameters of the evolution pattern of new languages and their reflection in SO.

The rest of the paper is organized as follows. Section~\ref{sec:Background and Data Collection} describes the background of our study and the data collection procedure. Section~\ref{sec:Dev discussions} reports the research questions about developers' discussion. Section~\ref{sec:Dev support} presents the research questions about the developers’ support to the three new languages. Section~\ref{sec:Implication} discusses the implications of our findings. Section~\ref{sec:validity} discusses the threats to validity. Section~\ref{sec:Related Works} presents the related work to our study, and Section~\ref{sec:conclusion} concludes the paper.


==> Sections/RQ5.tex <==
\subsection{RQ5. What are the characteristics of answer pattern for the languages?}
\label{RQ5}
\subsubsection{Motivation.} 
The developer base (programmer base) for the new languages grows over time. Initially, when there is a scarcity of developers/experts for a new language, a question may take time to be answered, and some questions may remain unanswered. With the increase in the number of experts and developers, continuous improvement is expected in these metrics. The change in answer pattern with respect to different aspects will be investigated in this RQ.

%New language developers look for answers/solutions to their problems on the QA site. To understand the growth of a new language and the effect of maturity, we must know the difference between the answer pattern of a new language and the pattern of a mature language. Since the problem/solution is one of the main features of the QA site, we also need to know if there is any significant difference in the answer pattern of any new language during the evolutionary period and its maturation period.

\subsubsection{Approach.} In SO, the community size and age of a language are most likely to influence the answer interval. The answer interval is likely to be decreased over time. To observe the expected change in intervals of new languages, we extracted several features from Stack Overflow like frequency of questions, questions without having any answer (no answer), questions having an accepted answer (accepted answer), and questions without an accepted answer (no accepted answer). To compare the growth, we plotted those features along with the features of one top-tier language (Java) and one mid-tier language (Python). Since Java is used in a wide range of projects, we have chosen it as a representative of top-tier languages. As the use of python has been steadily increasing in recent years, we have selected Python as a representative of mid-tier languages.

To check whether there is a significant difference in the answer pattern of a language during the evolutionary period and its maturation period, we have defined two states for languages according to the findings of Section \ref{RQ4}. (1) Evolving State: the language has just been released, it lacks experts and other resources in Stack Overflow, and (2) Matured State: the language has a stable release with a support community. The details of the stable date point are presented in Section \ref{RQ4}.


\begin{table}
%\resizebox{\textwidth}{!}{%
\caption{Duration of the evolving and matured state of new languages}
\begin{tabular}{|l|l|l|}
\hline
 Language & Evolving State & Matured State \\ \hline
% Swift & 01/09/14-30/04/16 & 01/05/16-31/12/17  \\ \hline
 Swift & September 2014-October 2016 & November 2016-December 2017  \\ \hline
 Rust & N/A & N/A \\ \hline
 Go & March 2012-June 2015 & July 2015-December 2017 \\ \hline
\end{tabular}%
%}
\label{table:States of languages}
\end{table}

After that, we have measured the median interval between the question and the first answer (first answer interval) and the interval between the question and the accepted answer (accepted answer interval) for each month for each of the languages. We hypothesized that there would be a significant difference in the answer interval between the two states of languages. To determine the appropriate method for testing the hypothesis, we conducted the Shapiro-Wilk test~\citep{SHAPIRO1965} and found that the distribution of the first answer interval does not follow a normal distribution. Since non-parametric tests do not assume any distribution, it is widely used in cases where the data does not follow the normal distribution~\citep{Mann1947}. Therefore, we used the non-parametric Man-Whitney U test to test the assumption that it takes longer to get the answer in the \emph{evolving state} than the \emph{matured state}.

It is expected that the number of unanswered questions will decrease with the evolution. To verify this assumption, we calculated the unanswered-question ratio for the new language for each month. By the unanswered question ratio, we mean the ratio of all questions and questions without any answers. We have defined the unanswered question ratio as,

$$ \text{Unanswered question ratio} = \dfrac{\sum \text{Unanswered questions}}{\sum \text{Questions}} $$


To compare the growth among the mature languages and new languages, we have collected the median time to get the first answer and the accepted answer. Furthermore, we have also completed an intra-language comparison of the first answer interval and accepted answer interval. Since the number of experts in a new language is relatively low, it is a general assumption that the new language will take longer to get accepted answers. So the accepted answer interval should be larger than the first answer interval.

\subsubsection{Results.}
The answer pattern of new and matured languages are presented in Figure~\ref{fig:Evolution of new languages}. It is clear from Figure~\ref{fig:Evolution of new languages} that the evolution pattern of Python is quite similar to Swift, while Java shows a different pattern compared to all three new languages. A natural deduction is that Java was released long before and was already a mature language prior to the inception of SO. Hence, the community interaction at the initial period of Java is missing in our dataset. On the other hand, although Python was also released long before the inception of SO, its use increased significantly after 2010~\citep{TIOBE:index}.

\begin{figure}
\includegraphics[scale=0.28]{figures/Evolution.eps} 
\caption{Question, No answer, Accepted answer, and No accepted answer count of languages in Stack Overflow}
\label{fig:Evolution of new languages}
\end{figure}


The result of the conjecture whether it takes longer in the \emph{evolving state} than the \emph{matured state} of their age to have the first answer and accepted answer is presented in Table~\ref{table:Mann-Whitney Test answer interval between states}.

\begin{table}[h]
\centering
\caption{Mann-Whitney U Test result for comparison of the first answer interval between matured and evolving state of new languages}
\begin{tabular}{|l|l|}
\hline
 Language & p value \\ \hline
 Swift & \textless 0.01  \\ \hline
 Rust & Not found \\ \hline
 Go &   \textless 0.01 \\ \hline
\end{tabular}%
\label{table:Mann-Whitney Test answer interval between states}
\end{table}

From the Mann-Whitney test result presented in Table~\ref{table:Mann-Whitney Test answer interval between states}, we have found that only the Swift and Go languages reject the null hypothesis which means that the difference is significant for Swift and Go languages.

\rifat{I think we don't need this. It is confusing because some of the mentioned topics are not in our previously shown topic list}.
\color{red}
There may be some differences between topics discussed in the evolving state and the matured state. To test the conjecture, we divided the questions of each language into two states and extracted 10 topics from each state. But the difference was not noticed between the topics. That is because while we are selecting a few topics from a large set, sub-topics grouped into common programming language topics. To overcome the problem, we extracted 50 topics from each state of each language with their percentage in that stage. If a topic does not appear at both stages, or if their percentage difference is greater than or equal to 2, then we considered that the topic belongs to that stage in which it is most commonly seen. We have tested with various threshold and selected two because otherwise, some topics which are common to all languages irrespective of the stage may appear. Now using this criterion we can identify the topic shift between states of languages.
\begin{enumerate}
\item \textbf{Topics of Swift Language in Evolving State:} During the evolving period, Swift developers mostly talked about language integration and equivalence. Since, in this period, the transition from Objective-C to Swift has just happened, developers were trying to transfer their codebase from Objective-C to Swift. Other popular topics in this state are the use of \emph{alamofire} (a HTTP library) and audio, video controller API of Swift.
\item \textbf{Topics of Swift Language in Matured State:} During the matured state, Swift developers are  mostly concerned about advanced features like ORM, advanced view controllers (segue), and threading. One thing prominent from the data that in matured state Swift developers are asking more questions related to game development such as different type of kits to handle 2D and 3D graphics (sprite kit, scene kit, etc.). The change might be associated with the availability of high-end phones in recent years~\citep{Aleem2016,Gavalas2011}.
\item \textbf{Topics of Go Language in Evolving State:} During the evolving state, Go developers discussed compiling issues, compiler path, data types, and type conversion. It seems that developers are trying to understand the syntax and usage of that language. Another common topic in this stage using simple HTTP, TCP, and socket server and encryption technology. As Go is mostly used in the server-side, developers are trying to identify Go's potential by deploying sample project or mimicing old project in the new language.

\item \textbf{Topics of Go Language in Matured State:} In the matured state, Go developers were concerned about HTTP web servers like Gin and  Martini, advanced features like ORM (GORM), and container deployment system Docker, Kubernetes. It is clear that developers are mostly concerned about delivering and deployment system  in this stage.
\end{enumerate}

\color{black}

\begin{figure}
\centering
\includegraphics[scale=0.38]{figures/UnansweredQuestionRatio.eps}
\caption{Unanswered-question ratio in Stack Overflow}
\label{fig:Unanswered-question ratio}
\end{figure}

The Unanswered question ratio of the languages is presented in Figure~\ref{fig:Unanswered-question ratio}. We have guessed that with time the Unanswered question ratio will gradually decrease. Figure ~\ref{fig:Unanswered-question ratio} shows the contrariwise scenery of our assumption. As the day goes by, the unanswered question ratio increases. In one sense, we can say that the answer pattern for new languages and matured languages are the same as in both cases, the unanswered question ration increases. However, we can observe two interesting phenomena from these results. First, the change ratio is smoother for matured language while it is notched for new languages except Swift. The reason for the jagged curve may be the absence of active expert developers. Inactive expert developers can change the ratio of the unanswered question by being active for a short time. That is why the curve for Go and Rust are jagged. Being the direct successor of Objective-C, Swift language has avoided this phenomenon. Second, Swift language starts its rise from a certain level caused by topic and question inheritance from Objective-C.

Figure~\ref{fig:Answer intervals} presents the median time to get the first answer and the accepted answer of new languages, a top-tier language (Java), and a mid-tier language (Python).
\begin{figure}
\begin{subfigure}{0.65\textwidth}
\centering
\hspace{-3cm}
\includegraphics[scale=0.38]{figures/AcceptedAnswerInterval.eps}
\caption{\textbf{Accepted answer}}
\label{fig:Accepted Answer interval}
\end{subfigure}
\begin{subfigure}{0.65\textwidth}
\centering
\hspace{-3cm}
\includegraphics[scale=0.38]{figures/FirstAnswerInterval.eps}
\caption{\textbf{First answer}}
\label{fig:First Answer interval}
\end{subfigure}
\caption{Comparison of median answer interval  of languages in Stack Overflow}
\label{fig:Answer intervals}
\end{figure}
Our intuition was that with maturity the time to get the first answer and the accepted answer would decrease. Figure~\ref{fig:Answer intervals} proves that our assumption is wrong. The answer intervals of Java is increasing in the long run which may be caused by various reason. However, a common reason behind the long answer interval of stack overflow questions is the inability to attract an expert developer to answer that question~\citep{Asaduzzaman2013}. However, we can observe steps in the accepted answer interval and the first answer interval of Python and Java. It points out that after a specific time, the answer interval increases. It is common in SO that matured communities often face repeated questions and \emph{hit and run}~\citep{DBLP:journals/corr/ChengDL14,SO:decay} problems cease the necessity of community collaboration significantly. The increment of answer interval for Python and Java language can be associated with that.

Time to get an accepted answer indirectly represents the growth of developers' expertise. From Figure~\ref{fig:Accepted Answer interval}, it is prominent that Rust has a comparatively longer accepted answer interval than the other two new languages. However, it is interesting that this is not true for the first answer interval. Go has a longer first answer interval than Rust. Hence, we can say that Rust's accepted answer interval is longer than Go but Go's first answer interval is longer than Rust. Longer accepted answer interval means the absence of expert developers. Thus, we can claim that Go developers receive the quality answer in the long run, but they have to wait a little longer as active support is absent. That means Stack overflow needs more \emph{active} Go developers and \emph{expert} Rust developers.

We have performed hypothesis testing on the accepted answer interval and the first answer interval of new languages to strengthen our claim. To find a suitable testing method for hypothesis testing, we have performed the Shapiro-Wilk test~\citep{SHAPIRO1965}. The Shapiro-Wilk test pointed out that the distribution is not normal. Thus we have performed a Mann-Whitney U test on first answer interval and accepted answer interval. The result is presented in Table~\ref{table:accepted-first u value}.
\input{Tables/accepted-first.tex}
From Table~\ref{table:accepted-first u value}, we can reject the null hypothesis for the first answer interval and the accepted answer interval of Go-Rust and Swift-Rust pair. It means that the difference between the first answer interval and the accepted answer interval of Rust-Go and Swift-Rust is statistically significant. It implies that our claim about the first and accepted answer intervals of Go and Rust is true.

\boxtext{In Stack Overflow, the unanswered question ratio increases regardless of the age of the language.}

\boxtext{In Stack Overflow, it takes significantly higher time to get the first answer in the evolving state than the matured state of a new language.}

\boxtext{In Stack Overflow, we found evidence that Go has comparatively less active community support, and Rust has a small number of expert developers.}


==> Sections/RQ6.tex <==
\subsection{RQ6. How likely are the questions of the three new languages answered by the developers of predecessor languages?}
\label{RQ6}
\subsubsection{Motivation.} If new languages share some common features with already well-established languages, the experts from that relevant established language are likely to contribute to the interested community of the new language. This may be crucial for the new languages because they do not have any community of their own at the initial stage. This research question will let us know about the details of the people who contributed significantly to the posts of the new languages, i.e., their prior experiences.

\subsubsection{Approach.} To answer this question, we need to find out which users are experts in answering queries of new languages and then find out their other areas of expertise. We defined \emph{expert developers} as those who have authored at least one accepted answer. First, we have identified expert developers for each language. We then collected tags of all the questions answered by the expert developers to look for other areas of expertise. After that, tags are sorted according to their frequency to get the most frequent tags.


% To answer this question, we have confined our search into the predecessor language of interest of the \emph{expert developers}. According to our definition,  \emph{expert developers} are those developers who have answered at least one accepted answer.
% To find the predecessor language of interest of the expert developers, we collected all the tags of the questions answered by expert developers and then sorted the tags according to their frequency to get the most frequent tags. 

\subsubsection{Results.}
The most frequent ten tags of answers by each language's expert developers are presented in Figure~\ref{fig:dev skills}.
% \input{Tables/answer_providers.tex}
\begin{figure}
\centering
\includegraphics[scale=0.5]{figures/Tagfrequency.eps}
\caption{Most frequent 10 tags answered by expert developers of new languages.}
\label{fig:dev skills}
\end{figure}

Rust experts mostly answered C and C++ questions previously. C++ is the predecessor language of Rust~\cite{Uzlu2017}. Hence, we can say developers expert in Rust are also expert in C and C++. We can infer that Rust is receiving contributions from the C and C++ community base in Stack Overflow. Developers expert in Swift have mostly answered the Java and Objective-C questions. Objective-C is considered the predecessor of the Swift language.

\boxtext{New languages are benefited from the community base of the predecessor language.}



==> Sections/ResearchSetting.tex <==
\section{Research Setting}
\label{sec:Research Setting}
This section introduces four research questions along with the motivation for this question. In this section, we will describe the research questions.

\subsection{Research Questions}
\noindent \textbf{RQ1.} What are the difficult topics in the questions of new languages in Stack Overflow?

\indent  Developers of new languages face problems that are rarely answered or get \emph{delayed answers}. By the \emph{delayed answer}, we imply that answer which is accepted by the user and received after the median answer interval of that month. We want to know about these questions so that special measures can be taken to answer this question.


\noindent  \textbf{RQ2.} Are the questions of new languages in Stack Overflow answered mostly by the developers of predecessor languages?

\indent Stack Overflow includes developers from a diverse domain. We are interested to see if there is a pattern that the experts in the predecessor of a new language mostly answers the questions of that language (e.g., Objective-C for Swift).


\noindent  \textbf{RQ3.} When can we expect the availability of adequate resource of the new languages in Stack Overflow?

\indent After the introduction of a new language, the resources of those languages may be absent in QA sites. Gradually the lackings will be met. We want to know the time interval after which we can expect the availability of these resources of new languages in Stack Overflow at a satisfactory level.

\noindent  \textbf{RQ4.} Is there any relation between the growth of a language and developers' activity pattern of that language?

\indent Stack Overflow has become one of the most prominent QA sites over the years. It has been used as a source to gain insight into developers' activity~\citep{Ahmed2017}. We can observe developers' activity from the frequency of question and answer in Stack Overflow and also from the number of developers and repositories of that language in GitHub. GitHub provides \emph{issue}~\citep{GithubIssue} to keep track of task, bug and feature request for a project. Most of the issues of a GitHub project are associated with bugs or feature request~\citep{Bissyande2013}. Therefore, it can be assumed that the solution to the issues leads to the advancement of the project. Hence, issues reflect the growth of the project. Moreover, every new release of a language implies the growth of that language. Thus, developers activity pattern after a new release of that language can also help to understand the relationship. We want to understand the relation between the growth of a programming language and developers' activity pattern.

\noindent  \textbf{RQ5.} What are the characteristics of answer pattern for new languages in Stack Overflow?

\indent With the evolution of a new language, the number of skilled developers increases. Being the most used programming related QA site, Stack Overflow is supposed to reflect that change. The increasing number of skilled developers may have its impact on answer patterns such as the expected interval of first and accepted answers, unanswered question ratio. By answer interval, we imply the delay between a question posted and an answer received. We want to know the characteristics of the answer pattern of new languages.



\iffalse


\noindent  \textbf{RQ6.} Is there any change over time in topics of Stack Overflow questions with the growth of the relevant language?

\indent Evolution of a language has many phases. These phases must have their footprint in the topics of the questions asked by the developers of the new languages. Hence, we want to know the topics of the questions asked by developers with respect to a timeline so that we can identify those phases.

\noindent \textbf{RQ7:} \emph{How do developers respond to the release of a new version of a language?}

\indent A new release of a language comes with a new and updated feature set. These updated or new features must have some impact over developer community. It may trigger new thread of question in Stack Overflow. We want to know the after effect of such release.
\fi


==> Tables/LDA_topic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{longtable}{|l|l|l|}
% \begin{tabular}{|l|l|l|}

\hline
Language              & Topic name & Top LDA words  \\ \hline
\multirow{6}{*}{Go}   & Problem in using library           & \textit{\begin{tabular}[c]{@{}l@{}}hql, gorm, mgo, grail,  dgo, beego,\\ hikari, error\_handling, groovy\end{tabular}}\\\cline{2-3}

                      & Serving request                    & \textit{\begin{tabular}[c]{@{}l@{}}grpc, server, ip\_address,\\request, testing, protocol,\\ socket, unmarshal, encryption\end{tabular}}\\\cline{2-3}
                      
                      & Go channel                         &  \textit{\begin{tabular}[c]{@{}l@{}}testing,
                      channel, mutex, thread,\\ http, syntax, lock, goroutine,\\ concurrency\end{tabular}} \\\cline{2-3}
                      
                      & Compilation problem                & \textit{\begin{tabular}[c]{@{}l@{}}gcompiler, go\_build, dwarf, cgo,\\ signed, flags, goreleaser, gocache, CI \end{tabular}}\\\cline{2-3}
                      
                      & Memory                             &   \textit{\begin{tabular}[c]{@{}l@{}}slice, memory\_allocation, network, io,\\ buffer, marshall, memory\_leak, pointer,\\ allocation\end{tabular}}\\\cline{2-3}
                      
                      & Migration Problem                  & \textit{\begin{tabular}[c]{@{}l@{}}data\_structure, server\_tech, language\_ equivalent,\\ compiler, syntax, clang integration,\\ convert, client\_communication, cgo\end{tabular}} \\\hline
\multirow{6}{*}{Rust} & Use of Struct        & \textit{\begin{tabular}[c]{@{}l@{}}syntax, lifetime,                                type\_conversion, algorithm,\\ clone, enclosed, filter, reference,\\                                           initialize\end{tabular}}\\\cline{2-3}

                      & Mutability           &  \textit{\begin{tabular}[c]{@{}l@{}}mutability, dref, scope,\\ moved\_value, closure, immutable,\\ FnMut\end{tabular}}\\\cline{2-3} 
                      
                      & Parallel execution   &  \textit{\begin{tabular}[c]{@{}l@{}}threads, sync, channel, rayon,\\ thread\_join, prelude, sequential, faster\end{tabular}}\\\cline{2-3}
                      
                      & Borrow mechanism     & \textit{\begin{tabular}[c]{@{}l@{}}borrow, frozen\_variable, ref, lifetime,\\ shadow, overlap, move, reuse, access\end{tabular}}\\\cline{2-3}
                      
                      & Use of Trait         & \textit{\begin{tabular}[c]{@{}l@{}}trait, static, dynamic, pointer,\\ polymorphism, unbox, generic, concrete,\\ conflict \end{tabular}}\\\cline{2-3}             
                      & Migration problem    & \textit{\begin{tabular}[c]{@{}l@{}}equivalent, compiler, syntax, jni,\\ extern, convert, pass, FFI,\\ wrap \end{tabular}}               \\\hline
\multirow{6}{*}{Swift}& UI                           &\textit{\begin{tabular}[c]{@{}l@{}}Ui,                                       view\_controller, animation,\\ layout, swiftUI, segue, graphics,\\ sprite, scene\_kit                           \end{tabular}}\\\cline{2-3}

                      & View Controller lifecycle    &\textit{\begin{tabular}[c]{@{}l@{}}hooks, cg\_size, appear,\\ disappear, will\_appear, deinit,\\ view, timer, dynamic \end{tabular}}\\\cline{2-3}
                      
                      & Mutability                   &\textit{\begin{tabular}[c]{@{}l@{}}collection, mutation, struct, let,\\ reference, mutable, modify, pointer,\\ unsafe\end{tabular}}\\\cline{2-3}
                      
                      & Data Handling                &\textit{\begin{tabular}[c]{@{}l@{}}database, json, parsing, persistence,\\ keychain, coredata, types, optional,\\ nested\end{tabular}}\\\cline{2-3}
                      
                      & Migration problem            &\textit{\begin{tabular}[c]{@{}l@{}}nullability, header, sub\_class,\\ swiftify , bridging, equivalence, object\_conversion,\\ protocol, dependency\end{tabular}}\\\cline{2-3}
                      
                      & Documentation clarification  &\textit{\begin{tabular}[c]{@{}l@{}}syntax, documentation, pragma\_mark,\\ xcode, comments, sdk, reference,\\ tutorial, apple-documentation\end{tabular}}\\\hline

         
% \end{tabular}
\caption{Topics discovered by LDA}
\end{longtable}

==> Tables/TagRelevance.tex <==

\begin{longtable}{|c|c|c|}
\caption{Significant and relevant tags of new languages used  to identify posts of new languages.}
\\ \hline
\textbf{$\alpha$ Value} & \textbf{$\beta$ Value} & \textbf{Set of Tags}\\ \hline

\multicolumn{3}{|c|}{Swift Language}                                                                                                            \\ \hline
0.01  & 0.01 & \begin{tabular}[c]{@{}c@{}}generics, parse.com, \\ dictionary, cocoa, uiwebview\end{tabular}                                     \\ \hline
0.01  & 0.02 & macos                                                                                                                            \\ \hline
0.01  & 0.03 & firebase                                                                                                                         \\ \hline
0.02  & 0.01 & \begin{tabular}[c]{@{}c@{}}uiviewcontroller, uiview,\\ uiimageview, uinavigationcontroller,\\ uiscrollview, uiimage\end{tabular} \\ \hline
0.02  & 0.02 & firebase-realtime-database                                                                                                       \\ \hline
0.02  & 0.1  & xcode                                                                                                                            \\ \hline
0.03  & 0.01 & \begin{tabular}[c]{@{}c@{}}uibutton, uitextfield,\\ uilabel, tableview,\\ mapkit, uitabbarcontroller\end{tabular}                \\ \hline
0.03  & 0.02 & core-data                                                                                                                        \\ \hline
0.03  & 0.06 & uitableview                                                                                                                      \\ \hline
0.03  & 0.55 & ios                                                                                                                              \\ \hline
0.04  & 0.01 & \begin{tabular}[c]{@{}c@{}}realm, cocoapods, avfoundation,\\ segue\end{tabular}                                                  \\ \hline
0.05  & 0.01 & protocols, nsuserdefaults                                                                                                        \\ \hline
0.05  & 0.02 & sprite-kit, uicollectionview                                                                                                     \\ \hline
0.06  & 0.01 & swift4, uicollectionviewcell                                                                                                     \\ \hline
0.07  & 0.5  & swift                                                                                                                            \\ \hline
0.12  & 0.02 & ios9                                                                                                                             \\ \hline
0.17  & 0.03 & alamofire                                                                                                                        \\ \hline
0.21  & 0.03 & xcode7                                                                                                                           \\ \hline
0.23  & 0.02 & ios10                                                                                                                            \\ \hline
0.39  & 0.06 & xcode8                                                                                                                           \\ \hline
1     & 0.01 & \begin{tabular}[c]{@{}c@{}}swift-extensions, swift2.3,\\ swift-package-manager,\\ swift2.1, swift2.2\end{tabular}                \\ \hline
1     & 0.02 & swift-protocols                                                                                                                  \\ \hline
1     & 0.03 & swift-playground                                                                                                                 \\ \hline
1     & 0.29 & swift2                                                                                                                           \\ \hline
1     & 0.63 & swift3                                                                                                                           \\ \hline
\multicolumn{3}{|c|}{Go Language}                                                                                                               \\ \hline
0.01  & 0.02 & hibernate, mongodb                                                                                                               \\ \hline
0.01  & 0.05 & json                                                                                                                             \\ \hline
0.02  & 0.01 & groovy, reflection                                                                                                               \\ \hline
0.02  & 0.02 & http                                                                                                                             \\ \hline
0.03  & 0.03 & google-app-engine                                                                                                                \\ \hline
0.04  & 0.01 & interface, google-cloud-datastore                                                                                                \\ \hline
0.04  & 0.02 & concurrency                                                                                                                      \\ \hline
0.05  & 0.03 & struct                                                                                                                           \\ \hline
0.13  & 0.01 & grpc                                                                                                                             \\ \hline
0.13  & 0.1  & grails                                                                                                                           \\ \hline
0.15  & 0.01 & grails-2.0                                                                                                                       \\ \hline
0.2   & 0.01 & unmarshalling                                                                                                                    \\ \hline
0.21  & 0.02 & slice                                                                                                                            \\ \hline
0.38  & 0.01 & grails-domain-class                                                                                                              \\ \hline
0.41  & 0.01 & channel                                                                                                                          \\ \hline
0.86  & 0.01 & go-templates                                                                                                                     \\ \hline
0.91  & 0.01 & beego                                                                                                                            \\ \hline
0.97  & 0.01 & mgo                                                                                                                              \\ \hline
0.99  & 0.01 & gorilla                                                                                                                          \\ \hline
1     & 0.01 & cgo, go-gorm                                                                                                                     \\ \hline
1     & 0.02 & goroutine                                                                                                                        \\ \hline
1     & 0.1  & gorm                                                                                                                             \\ \hline
1     & 0.89 & go                                                                                                                               \\ \hline
\multicolumn{3}{|c|}{Rust Language}                                                                                                             \\ \hline
0.01  & 0.01 & \begin{tabular}[c]{@{}c@{}}types, reference,\\ enums, pattern-matching,\\ hashmap\end{tabular}                                   \\ \hline
0.01  & 0.02 & vector, struct                                                                                                                   \\ \hline
0.01  & 0.03 & generics                                                                                                                         \\ \hline
0.02  & 0.01 & slice                                                                                                                            \\ \hline
0.02  & 0.02 & iterator, macros                                                                                                                 \\ \hline
0.03  & 0.01 & future                                                                                                                           \\ \hline
0.03  & 0.02 & closures                                                                                                                         \\ \hline
0.07  & 0.01 & mutable                                                                                                                          \\ \hline
0.21  & 0.02 & ffi                                                                                                                              \\ \hline
0.24  & 0.04 & traits                                                                                                                           \\ \hline
0.3   & 0.01 & ownership                                                                                                                        \\ \hline
0.66  & 0.06 & lifetime                                                                                                                         \\ \hline
0.87  & 0.01 & hyper                                                                                                                            \\ \hline
1     & 0.01 & \begin{tabular}[c]{@{}c@{}}serde, borrowing,\\ rust-tokio, rust-crates\end{tabular}                                              \\ \hline
1     & 0.03 & borrow-checker                                                                                                                   \\ \hline
1     & 0.04 & rust-cargo                                                                                                                       \\ \hline
1     & 1    & rust                                          \label{appendix:tagrelevance}                                                                           \\ \hline


\end{longtable}


==> Tables/accepted-first.tex <==
\iffalse
\begin{table}
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
        Go & Rust &  p value \\ \hline
        Accepted Answer Interval  &  First Answer Interval     &  < 0.01 \\ \hline
        First Answer Interval     &  Accepted Answer Interval  &  < 0.01  \\ \hline
\end{tabular}
%}
\caption{Mann-Whitney U test result for the comparison of accepted answer time and first answer time of Go and Rust language}
\label{table:accepted-first u value}
\end{table}
\fi



\begin{table}
\caption{Mann-Whitney U test result for the comparison of accepted answer time and first answer time of Go and Rust language}
\begin{tabular}{|l|c|c|c|}
\hline
\multirow{2}{*}{Test Subject}                                   & \multicolumn{2}{c|}{Language}                                     & \multicolumn{1}{l|}{\multirow{2}{*}{p value}} \\ \cline{2-3}
                                                                & \multicolumn{1}{l|}{Language 1} & \multicolumn{1}{l|}{Language 2} & \multicolumn{1}{l|}{}                         \\ \hline
\multirow{3}{*}{First Answer Interval}                          & Go                              & Swift                           &     0.158                                          \\ \cline{2-4} 
                                                                & Go                              & Rust                            &    \textless 0.01                                           \\ \cline{2-4} 
                                                                & Swift                           & Rust                            &      \textless 0.01                                         \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Accepted Answer Interval}} & Go                              & Swift                           &        0.389                                       \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                          & Swift                           & Rust                            &         \textless 0.1                                      \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                          & Go                           & Rust                            &           \textless 0.01                                    \\ \hline
\end{tabular}

\label{table:accepted-first u value}
\end{table}



==> Tables/answer_providers.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|l|l|}
    \hline
    Developers & Tags in order of occurrence\\ \hline
    
    \multirow{2}{*}{Swift Developers}
    &iOS\\&Java\\&Objective-C\\&Swift\\&JavaScript\\&Android\\&iPhone\\&Php\\&C++\\&C\# \\ \hline
    
    \multirow{2}{*}{Go Developers}
    &Java  \\ &JavaScript\\ &Python \\&C++\\&Php\\&C\#\\&MySQL\\&C\\&Regex\\&JQuery \\ \hline
    
    \multirow{2}{*}{Rust Developers}
    &C++\\&C\\&Java\\&Python \\& Rust\\ &Ruby\\ &C\# \\ &Haskell \\ &JavaScript 	\\ &Linux\\ \hline
    


\end{tabular}
\end{center}
\caption{Most frequent 10 tags answered by expert developers of new languages.}
\label{table:Dev skills}
\end{table}

==> Tables/equation.tex <==
\begin{table*}[htbp]
  \centering
  \begin{tabular}{l}
    \eqrow{Q=\big\{All\quad Questions\quad of\quad a\quad month  \big\}}
    \eqrow{A=\big\{All\quad answers\quad of\quad questions\quad in\quad Q\quad where \quad creation\quad date\quad is\quad within\quad 24 \quad hour\quad of\quad Q \big\} }
    \eqrow{C=\big\{All\quad comments\quad of\quad Q\quad within\quad 24\quad hour\quad of\quad Q\big\} \cup  \big\{All\quad comments\quad of\quad A\quad within\quad 24\quad hour\quad of\quad A\big\}}
    \eqrow{AA=\big\{All\quad accepted\quad answers\quad of\quad Q\quad where creation\quad date\quad is\quad within\quad 24\quad hour\quad of\quad Q \big\}}
    \eqrow{T(x)=Creation\quad date\quad time\quad of\quad item\quad x }
    \eqrow{{Interaction \quad score=}\left[\dfrac{ \sum_{Q_i\in Q}Q_i+ \sum_{A_i\in A}A_i+\sum_{C_i\in C}C_i}{\sum_{Q_i\in Q}Q_i}\right] \hspace{10em}}
    \eqrow{{Score=}\left[\dfrac{ \sum_{Q_i\in Q}\sum_{\substack{Q_v\in Votes\: of\: Q_i\\ Q_v \leq T(Q_i)+24}}Q_v  +\sum_{A_i\in A}\sum_{\substack{A_v\in Votes\: of\: A_i\\ A_v \leq T(A_i)+24}}A_v + \sum_{AA_i\in AA}\sum_{\substack{AA_v\in Votes\: of\: AA_i\\ AA_v \leq T(AA_i)+24}}AA_v}{\sum_{Q_i\in Q}Q_i}\right]}
  \end{tabular}
\end{table*}

==> Tables/go_topic.tex <==



\begin{table}[]
\begin{tabular}{|l|l|}
\hline
Time Duration & Topics \\ \hline
\multirow{1}{*}{Jul,2008 - Jan,2009} & Grail,Hibernate\\ \hline
\multirow{2}{*}{Jan,2009 - Jul,2009} & Persistency,Backward comptibility,Session,Concurrency,Grail,\\ & Orm,Hibernate\\ \hline
\multirow{2}{*}{Jan,2010 - Jul,2010} & Pointer,Hql,Goinstall,Git issue,Grail idiomatic,Inheritance,\\ & Interface,Object nstance,Haskell emulate,Hibernate,Gorm,Network,\\ & Database connection,Generic data structure,Hash,Rsa librray,\\ & Python execute\\ \hline
\multirow{2}{*}{Jan,2011 - Jul,2011} & Hibernate,Grail,Gorm,Groovy,Ssh,Spring,Scala emulate,Exception handling,\\ & Drool,Async loading,Concurrency,Pointer,Hql,Enumerator,Serialization,\\ & Security,Object reference\\ \hline
\multirow{2}{*}{Jul,2011 - Jan,2012} & Oracle,Pipe,Wildcard,Rpc,Bitcoin,Go make,Os support,Interpretor,\\ & Ide,Grail,Groovy,Android,Gorm\\ \hline
\multirow{2}{*}{Jan,2012 - Jul,2012} & Data type,Gorm,Pipe,Hql,Cache,Hibernate,Exception handling,Inheritance,\\ & Go routine,Memory access,Cgo,Session,Sql,Go idiomatic ,Groovy,\\ & Python\\ \hline
\multirow{2}{*}{Jul,2012 - Jan,2013} & Hibernate,App engine,Session,Grail,Go routine,Database driver,\\ & Google app engine,Os dependency,Hql,Gorm,Disk access,Interface,\\ & Pointer,Struct,Cgo\\ \hline
\multirow{2}{*}{Jan,2013 - Jul,2013} & Cgo,Google app engine,Go idiomatic,Go panic,Groovy,Database connection,\\ & Oauth librray,Override,Pointer,Testing suite,Gorm,Grail,Xml parsing,\\ & Hibernate,Server creation\\ \hline
\multirow{2}{*}{Jul,2013 - Jan,2014} & Xml,Context storing,Hibernate,Cgo,Google app engine,Go routine,\\ & Grail,Gorilla,Regex,Databse transaction,Gorm,Sql,Go panic\\ \hline
\multirow{2}{*}{Jan,2014 - Jul,2014} & Gorm,Image  library,Xml parsing,Documentation,Parameter passing,\\ & Groovy,Go routine,Regex,Serialization,Grail,Server creation,\\ & Network protocol,Google app engine,Hibernate,Automated testing,\\\\ \hline
\multirow{2}{*}{Jul,2014 - Jan,2015} & Webframework,Argument passing,Gorm,Go martini,Sql,Inheritance,\\ & Disk access,Network protocol,Grail,Json parser,Database operation,\\ & Installation issue,Gorilla,Google app engine,Orm,Docker,Databse transaction,\\ & Go routine,Json parsing\\ \hline
\multirow{2}{*}{Jan,2016 - Jul,2016} & Xml parser,Goroutine,Dtaabse driver,Gorilla,Network programming,\\ & Database connection,Network protocol,Restful service,Interface,\\ & Serever configuration,Runtime error,Compilation issue,Dependency tool,\\ & Oauth librray,Gorm,Syntax,Service creation\\ \hline
\multirow{2}{*}{Jul,2016 - Jan,2017} & Grail,Go routine,Server,Database driver,Android,Serialization,\\ & Authentication protocol,Pointer,Cgo,Web framework,Concurrency,\\ & Session,Interface\\ \hline
\multirow{2}{*}{Jan,2017 - Jul,2017} & Network programming,Go routine,Unmarshal,Server,Grpc,Static variable,\\ & Gorilla,Database,Grail,Mux,Beego framework,Runtime,Debugging,\\ & Docker,Gorm\\ \hline
\multirow{2}{*}{Jul,2017 - Jan,2018} & Databse driver,Go routine,Ssh,Grail,Thread safety,Web framework,\\ & Python emulate,Concurrency,Json parsing,Network programming,\\ & Interface,Gorm,Ide,Regex,Cgo,Grpc protocol\\ \hline

\end{tabular}
\caption{Go topics}
\label{table:Go topics}
\end{table}

==> Tables/language_topics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\centering
\caption{Top six difficult topics of new languages (\ra{same topics are colored with the same color})}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Swift} & \textbf{Go}  & \textbf{Rust} \\ \hline
User Interface  & Library Integration & Use of Struct \\ \hline
View Controller Lifecycle & Webserver & \cellcolor[HTML]{999903} Mutability\\ \hline
\cellcolor[HTML]{999903}Mutability & Go Channel  & Parallel Execution\\ \hline
Data Handling  & Compilation Problem  & Borrow Mechanism \\ \hline
\cellcolor[HTML]{4793A5}Migration & Memory Handling  & Use of Trait \\ \hline
Foundation Kit  & \cellcolor[HTML]{4793A5}Migration & \cellcolor[HTML]{4793A5}Migration \\ \hline
\end{tabular}
\label{table:language topics}
\end{table}

==> Tables/rust_topic.tex <==
\begin{table}[]
\begin{tabular}{|l|l|}
\hline
Time Duration & Topics \\ \hline
\multirow{1}{*}{Jul,2010 - Jan,2011} & Typestate\\ \hline
\multirow{2}{*}{Jan,2012 - Jul,2012} & Rust ffi,Lisp lang,Database lib,Network programming,Digital signature,\\ & Lisp emulator\\ \hline
\multirow{2}{*}{Jul,2012 - Jan,2013} & Pointer,Interface,Aliasing,Memory leakage,Benchmark,Parsing,\\ & Recursive depth\\ \hline
\multirow{2}{*}{Jan,2013 - Jul,2013} & Crate,Operator overloading,Parser,Compilation issue,Rust pipes,\\ & Graphics programming,Generics,Rust pipe,Network protocol,Rust ffi,\\ & Thread,Syntax,Extern,Windows programming,Stack size\\ \hline
\multirow{2}{*}{Jul,2013 - Jan,2014} & Database connection,Concurrency,Enum,Varibale passing,Syntax lambda,\\ & Stream,Pointer,Thread,Inheritance,Mutable datastructure,Network programming,\\ & Rust modules,Unicode handling,Borrow package,Stdin,Database module,\\ & Libc\\ \hline
\multirow{2}{*}{Jan,2014 - Jul,2014} & Installation issue,Rust idiomatic ,Streaming,Crate,Macro,Shell access,\\ & Enumerator,Generic pointer,Unicode value,Socket in ffi,Rust box,\\ & Rust trait,Inheritance,Network,Object creation\\ \hline
\multirow{2}{*}{Jul,2014 - Jan,2015} & Dereferencing,Macro,Pointer,Struct,Thread,Generic object,Data structure,\\ & Network programming,Annotation,Cargo,Enumerator,Rust trait,Rust ffi,\\ & Argument passing,Immutable struct,Rust box\\ \hline
\multirow{2}{*}{Jan,2015 - Jul,2015} & Rust borrow,Box,Trait,Rust arc,Stack,Mutablity,Thread lifetime,\\ & Rust fnonce,Network stream,Enumerator,Rustc dependency,Dynamic linking librray,\\ & Threads,Macro,Rust borrow,Cargo,Rust idiomatic\\ \hline
\multirow{2}{*}{Jul,2015 - Jan,2016} & Regex,Windows dependency,Immutable varibales,Thread,Rust compiler,\\ & Mutability,File parser,I/o,Rustc,Rust ffi,Impl block,Macro,Object lifetime,\\ & Serialization,Generic trait,Struct,Rust trait\\ \hline
\multirow{2}{*}{Jan,2016 - Jul,2016} & Concurrency,Data type,Threads,Memory issue,Syntax,Documentation,\\ & Dynamic arguments,Variable type,Library,Pointer,Function parameter,\\ & Standard library,Standard i/o,Disk access,Data type,Variable mutability,\\ & Rust box,Iterator,Parameter passing\\ \hline
\multirow{2}{*}{Jul,2016 - Jan,2017} & Static variable,Immutable type,Rust ffi,Rust box,Llvm,Crate,\\ & Generic,Object reference,Macro,Cargo,Iterator,Heap,Inheritance,\\ & Docker,Rust trait,Memory reference,Mutable variable\\ \hline
\multirow{2}{*}{Jan,2017 - Jul,2017} & Orm,Dynamic linking,Xml parsing,I/o librray,Documentation,Cfg,\\ & Pointer,Crates,Rust serde,Rust trait,Struct,Cargo,Dereferencing,\\ & Rustc,Heap,Crate,Mutable,Box\\ \hline
\multirow{2}{*}{Jul,2017 - Jan,2018} & Macro,Rust panic,Rust box,Cargo,Compiling issue,Object lifetime,\\ & Network programming,Rust idiomatic,Crate,Thread safety,Syntax,\\ & Trait,Streaming library,Generic data structure,Standard referenece,\\ & Thread lifecycle\\ \hline

\end{tabular}
\caption{Rust topics}
\label{table:Rust topics}
\end{table}

==> Tables/swift_topic.tex <==
\begin{table}[]
\begin{tabular}{|l|l|}
\hline
Time Duration & Topics \\ \hline


\multirow{1}{*}{Jan,2011 - Jul,2011} & Service,Date parser,Ui\\ \hline
\multirow{2}{*}{Jul,2011 - Jan,2012} & Ui,Context,Process binding,Regex,Request lib,Service documentation,\\ & Xml\\ \hline
\multirow{2}{*}{Jan,2012 - Jul,2012} & Ui,Camera sdk,Audio documentation,String operation,Swift segue,\\ & Build error,Notification service,Spring,Xcode,Network programming,\\ \hline
\multirow{2}{*}{Jul,2012 - Jan,2013} & Sdk documentation,Sdk backward compatibility,Tutorial,Ui object,\\ & Ui,Swift segue,Design pattern,Sdk\\ \hline
\multirow{2}{*}{Jul,2013 - Jan,2014} & Watchos,Swift segue,Ndk,Ui,Rsa,Dependency management,Animation,\\\\ \hline
\multirow{2}{*}{Jul,2014 - Jan,2015} & Ui,Json parsing,Argument passing,Generic,Framework,Compilation error,\\ & Xcode,Os dependency,Session\\ \hline
\multirow{2}{*}{Jan,2015 - Jul,2015} & Framework,Ui,Thread,Spritekit,Git,Camera access,Network protocol,\\ & Gesture detection\\ \hline
\multirow{2}{*}{Jul,2015 - Jan,2016} & Spritekit,Exception handling,Ui,View controller,Xcode,Framework,\\ & Network,Api documentation,Parsing\\ \hline
\multirow{2}{*}{Jan,2016 - Jul,2016} & Object serialization,Framework,Ui,Realm,Protocol,Watch framework,\\ & Firebase,Session\\ \hline
\multirow{2}{*}{Jan,2017 - Jul,2017} & Media documentation,Watchos,Date parsing,Ui,Animation,Spritekit,\\ & Xcode,Stream,View controller,Firebase,Thread,Facebook sdk,Error,\\ \hline
\end{tabular}
\caption{Swift topics}
\label{table:Swift topics}
\end{table}

==> Tables/topic_difficulty_previous.tex <==
\begin{table}[htbp]
\centering
\begin{subtable}[htbp]{1\textwidth}
\centering
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c|}{Topic}                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Posts w/o\\ Accepted (\%)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Median\\ Time (m)\end{tabular}} \\ \hline

\multicolumn{1}{l|}{Migration}                   & \multicolumn{1}{r|}{59.6}                                                              & 95                                                                            \\
\multicolumn{1}{l|}{Documentation Clarification} & \multicolumn{1}{r|}{52.2}                                                              & 43                                                                            \\
\multicolumn{1}{l|}{Graphics}                    & \multicolumn{1}{r|}{51.2}                                                              & 58                                                                            \\
\multicolumn{1}{l|}{View Controller Lifecycle}   & \multicolumn{1}{r|}{51.1}                                                              & 36                                                                            \\
\multicolumn{1}{l|}{Data Handling}               & \multicolumn{1}{r|}{49.8}                                                              & 30                                                                            \\
\multicolumn{1}{l|}{Mutability}                  & \multicolumn{1}{r|}{49.4}                                                              & 32                                                                            \\
\multicolumn{1}{l|}{Foundation Kit}              & \multicolumn{1}{r|}{49.3}                                                              & 35                                                                            \\
\multicolumn{1}{l|}{User Interface}              & \multicolumn{1}{r|}{48.7}                                                              & 36                                                                            \\
\multicolumn{1}{l|}{Portable Database}           & \multicolumn{1}{r|}{47.8}                                                              & 50                                                                            \\
\multicolumn{1}{l|}{Type Conversion}             & \multicolumn{1}{r|}{36.5}                                                              & 23                                                                            \\ \hline
\end{tabular}
\caption{Per topic difficulty of Swift language.}
\label{table:topic_difficulty_swift}
\end{subtable}

\begin{subtable}[htbp]{1\textwidth}
\centering
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c|}{Topic}                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Posts w/o\\ Accepted (\%)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Median\\ Time (m)\end{tabular}} \\ \hline

\multicolumn{1}{l|}{Request Serving}             & \multicolumn{1}{r|}{46.4}                                                              & 97                                                                            \\
\multicolumn{1}{l|}{Migration}                   & \multicolumn{1}{r|}{46.4}                                                              & 111                                                                           \\
\multicolumn{1}{l|}{Compilation Problem}         & \multicolumn{1}{r|}{44.8}                                                              & 69                                                                            \\
\multicolumn{1}{l|}{Library Problem}             & \multicolumn{1}{r|}{39.8}                                                              & 60                                                                            \\
\multicolumn{1}{l|}{I/O Operation}               & \multicolumn{1}{r|}{37.4}                                                              & 47                                                                            \\
\multicolumn{1}{l|}{Memory Handling}             & \multicolumn{1}{r|}{36.1}                                                              & 41                                                                            \\
\multicolumn{1}{l|}{Go Channel}                  & \multicolumn{1}{r|}{33.8}                                                              & 37                                                                            \\
\multicolumn{1}{l|}{Unmarshalling/Marshalling}   & \multicolumn{1}{r|}{29}                                                                & 26                                                                            \\
\multicolumn{1}{l|}{Type Conversion}             & \multicolumn{1}{r|}{26.9}                                                              & 22                                                                            \\
\multicolumn{1}{l|}{Pointer}                     & \multicolumn{1}{r|}{26.6}                                                              & 22                                                                            \\ \hline
\end{tabular}
\caption{Per topic difficulty of Go language.}
\label{table:topic_difficulty_go}
\end{subtable}
\end{table}

\begin{table}
\ContinuedFloat
\centering
\begin{subtable}[htbp]{1\textwidth}

\centering
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c|}{Topic}                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Posts w/o\\ Accepted (\%)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Median\\ Time (m)\end{tabular}} \\ \hline

\multicolumn{1}{l|}{Parallel Execution}          & \multicolumn{1}{r|}{36.2}                                                              & 111                                                                           \\
\multicolumn{1}{l|}{Cargo}                       & \multicolumn{1}{r|}{34.8}                                                              & 66                                                                            \\
\multicolumn{1}{l|}{Migration Problem}           & \multicolumn{1}{r|}{28.2}                                                              & 55                                                                            \\
\multicolumn{1}{l|}{Database}                    & \multicolumn{1}{r|}{27.9}                                                              & 56                                                                            \\
\multicolumn{1}{l|}{Borrow Mechanism}            & \multicolumn{1}{r|}{27}                                                                & 28                                                                            \\
\multicolumn{1}{l|}{Mutability}                  & \multicolumn{1}{r|}{27}                                                                & 38                                                                            \\
\multicolumn{1}{l|}{Use of Trait}                & \multicolumn{1}{r|}{26.9}                                                              & 39                                                                            \\
\multicolumn{1}{l|}{Generic Coding}              & \multicolumn{1}{r|}{26.5}                                                              & 41                                                                            \\
\multicolumn{1}{l|}{Mutex}                       & \multicolumn{1}{r|}{26}                                                                & 45                                                                            \\
\multicolumn{1}{l|}{Use of Struct}               & \multicolumn{1}{r|}{20.9}                                                              & 35                                                                            \\ \hline
\end{tabular}

\caption{Per topic difficulty of Rust language.}
\label{table:topic_difficulty_rust}
\end{subtable}

\caption{Topic difficulty of new languages.}
\label{table:topic_difficulty}
\end{table}


